Too Big to Fail? Active Few-Shot Learning Guided Logic Synthesis

Generating sub-optimal synthesis transformation sequences ("synthesis recipe") is an important problem in logic synthesis. Manually crafted synthesis recipes have poor quality. State-of-the art machine learning (ML) works to generate synthesis recipes do not scale to large netlists as the models need to be trained from scratch, for which training data is collected using time consuming synthesis runs. We propose a new approach, Bulls-Eye, that fine-tunes a pre-trained model on past synthesis data to accurately predict the quality of a synthesis recipe for an unseen netlist. This approach on achieves 2x-10x run-time improvement and better quality-of-result (QoR) than state-of-the-art machine learning approaches.

==> 08_biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1.2in,height=1.5in,clip,keepaspectratio]{bio/animeshBasakChowdhury.png}}]{Animesh Basak Chowdhury} is a Ph.D. candidate at the NYU Centre for Cybersecurity, where he works in the area of machine learning for Electronics Design Automation and security testing. He received his MS in Computer Science from Indian Statistical Institute in 2016. Prior to joining the Ph.D. program, he spent three years as a researcher at Tata Research Development and Design Centre (TRDDC), India, where he was primarily working in the area of formal verification and security testing. He has won several awards and recognition in International Software Verification and Testing Competitions (SV-COMP, TEST COMP, and RERS-Challenge).

\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/BT-journal.jpeg}}]{Benjamin Tan}
(S'13-M'18) received the BE(Hons) degree in Computer Systems Engineering, in 2014, and the Ph.D. degree, in 2019, both from the University of Auckland. Since 2019, he has been a Research Assistant Professor working in the NYU Center for Cybersecurity, New York University, NY, USA. His research interests include hardware security, electronic design automation, and machine learning. He is a member of the IEEE and ACM. 
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/sg-photo-journal.jpg}}]{Siddharth Garg}
 received the B.Tech. degree in electrical engineering from IIT Madras and the Ph.D. degree in electrical and computer engineering from Carnegie Mellon University, in 2009. He was an Assistant Professor with the University of Waterloo, from 2010 to 2014. In 2014, he joined New York University (NYU) as an Assistant Professor. His general research interest includes computer engineering, more particularly secure, reliable, and energy-efficient computing. He was a recipient of the NSF CAREER Award, in 2015. 
% He received paper awards from the IEEE Symposium on Security and Privacy (S\&P), in 2016, the USENIX Security Symposium, in 2013, the Semiconductor Research Consortium TECHCON, in 2010, and the International Symposium on Quality in Electronic Design (ISQED), in 2009. 
 %He also received the Angel G. Jordan Award from the Electrical and Computer Engineering (ECE) Department, Carnegie Mellon University, for outstanding dissertation contributions and service to the community.
 \end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.25in,clip,keepaspectratio]{bio/rkarri.jpg}}]{Ramesh Karri} 
  is a Professor of ECE at New York University. He co-directs the NYU Center 
for Cyber Security (http://cyber.nyu.edu). He founded the Embedded Systems Challenge (https://csaw.engineering.nyu.edu/esc), the annual 
red team blue team event. He co-founded Trust-Hub (http://trust-hub.org). 
Ramesh Karri has a Ph.D. in Computer Science and 
Engineering, from the UC San Diego and a B.E in ECE from Andhra University. His 
research and education activities in hardware cybersecurity include trustworthy 
ICs; processors and cyber-physical systems; security-aware computer-aided 
design, test, verification, validation, and reliability; nano meets security; 
hardware security competitions, benchmarks, and metrics; biochip security; 
additive manufacturing security. He  published over 250 articles in leading 
journals and conference proceedings. Karri's work on hardware cybersecurity 
received best paper nominations (ICCD 2015 and DFTS 2015) and awards (ACM TODAES 
2018, ITC 2014, CCS 2013, DFTS 2013 and VLSI Design 2012). He received the 
Humboldt Fellowship and the NSF CAREER Award. He is the editor-in-chief of ACM JETC and serve(d)s  
on the editorial boards of IEEE and ACM Transactions (TIFS, TCAD, 
TODAES, ESL, D\&T, JETC). He was an IEEE Computer Society Distinguished 
Visitor (2013-2015). He served on the Executive Committee of the IEEE/ACM 
DAC leading the Security\@DAC initiative (2014-2017). 
He served as program/general chair of conferences and serves on program committees. 
He is a Fellow of the IEEE for leadership and contributions to Trustworthy Hardware.
\end{IEEEbiography}

==> images/mainflow.tex <==
% \section{Diagrammatic view of Multisketch operations}\label{app:mainflow}  

% A user registers with a user id $\u$ and a vector of biometric templates
% $\mvec=\mvecss{\mlen}$. Multisketch uses two databases $\dbid$ and $\dbmsg$\@,
% where $\dbid$ contains user id $\u$ and the corresponding helper data
% $\sketchval$, and $\dbmsg$ contains the random permutation of the templates
% registered so far. Highlighted are the entries corresponding to a user $\u_4$
% with templates $\mvec_4=\mvec_{41}\ldots\mvec_{4\mlen}$.% and helper
%     % data $\sketchval_4$.
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
    >=stealth,
    node distance=2cm,
    database/.style={
      cylinder,
      cylinder uses custom fill,
      cylinder body fill=black!25!white,
      cylinder end fill=black!25!white,
      shape border rotate=90,
      aspect=0.25,
      minimum width=2em,
      minimum height=2em,
      draw
    },
    func/.style={
      rectangle,
      fill=red!25!white,
      minimum width=1cm,
      minimum height=1em,
      draw
    },
    cell/.style={
      rectangle,
      draw=black!50!white
    }
    ]
    \node (user) at (0, 0) {User};
    \node[func, right of=user, right=-1.1em, above=3em] (msketch) {$\MS$}; 
    \draw[below of=msketch, dashed, anchor=west] (.85,0.55) rectangle (5.9,-1.2); 
    \node[func, below of=msketch, anchor=east, below=1.95cm,fill=red!10!white,dashed] (mrecover) {$\MRec$};
    % \node[database, right of=user, anchor=south, above=1em, right=2cm] (db1) {$\dbid$};
    \matrix (db1) [right of=user, anchor=south, below=2pt, right=-0.1cm, 
    matrix of math nodes,
    column sep = -\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}}, 
    column 2/.style={nodes={cell}}, 
    anchor=west] {
      \u_1 & \sketchval_1\\
      \u_2 & \sketchval_2\\
      \u_3 & \sketchval_3\\
      |[draw,fill=blue!20]|\u_4 & |[draw,fill=blue!20]|\sketchval_4\\
    };
    \node[left of=db1, anchor=east,right=1.1cm] {$\dbid$};
    \matrix (db2) [right of=db1, left=25pt, matrix of math nodes,
    column sep = 2\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}},
    column 2/.style={nodes={cell}}, 
    column 3/.style={nodes={cell}}, 
    column 4/.style={nodes={cell}}, 
    column 5/.style={nodes={cell}}, 
    anchor=west] {
      \mvec_{21} &\mvec_{12} & |[draw,fill=blue!20]|\mvec_{43} &  & \mvec_{3\mlen} \\
      |[draw,fill=blue!20]|\mvec_{41} &\mvec_{32} & \mvec_{33} & |[draw=white]|\ldots & \mvec_{2\mlen} \\
      \mvec_{11} &|[draw,fill=blue!20]|\mvec_{42} & \mvec_{23} &  & \mvec_{1\mlen} \\
      \mvec_{31} &\mvec_{22} & \mvec_{13} & & |[draw,fill=blue!20]|\mvec_{4\mlen} \\
    };
    \node[left of=db2, left=-4pt] {$\dbmsg$};

    % \node[database,right of=db1] (db2) {$\dbmsg$};
    \node[func,below of=db1,anchor=north,above=8pt,left=8pt] (gu) {GetUser};
    \node[func,right of=gu,anchor=east,right=-5pt] (fm) {FindMatches};
    \node[func,below of=db1,anchor=east,below=2em,right=-3pt] (recover) {Recover};

    \draw[->,blue!50,thick] (user.north) |- node[black,near end,above]{$u, \mvec$} node[black,near end,below,font=\small]{register} 
    (msketch.west);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$u, \sketchval$} (db1);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$\mvec$} (db2);

    \draw[->,blue!50,thick] (user.south) |- ++(1,-0.9) node[black,near end,above]{$u, \mvectilde$} node[black,near end,below,font=\small]{login}   -| node[black,left,near end]{$u$}
    (gu.north);
    \draw[->,blue!50,thick] (user.south) |- ++(0,-0.9)  -- ++(3.1,0) |- node[black,near end, above]{$\mvectilde$}
    (fm.west);
    \draw[->,blue!50,thick] (db1.south) |- node[black,near end,above]{} (gu.east);
    \draw[->,blue!50,thick] (db2.south) |- node[black,near end,above]{} (fm.east);
    \draw[->,blue!50,thick] (gu.south) |- node[black,near end,above]{$\sketchval$} (recover.west);
    \draw[->,blue!50,thick] (fm.south) |- node[black,near end,above]{$\mvec'$} (recover.east);    
    \draw[->,blue!50,line width=2pt] (recover.south) -- node[black,near end,right]{$\mvec$ or $\bot$} ++(0, -0.65);
  \end{tikzpicture}
  % \rcnote{Rough sketch of the flow of the \biosketch.} 
  \caption{Diagram of multisketch as a part of an authentication service. 
  }
  \label{fig:mainflow}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> simulated-annealing-table.tex <==
\begin{table*}[htbp]
\centering
\footnotesize
\caption{Quality of synthesized netlists from using recipes found with various evaluators in simulated annealing. 
% Designs from \cite{iccad_2021,mlcad_abc,drills} and other large benchmarks.
$B$: Actual synthesis, $S$: Standalone predictor trained on 50 recipes, $ZS$: Zero-shot predictor, $F^R$: Fine-tuned predictor using random recipes, $F^A$: Fine-tuned predictor using active learning. 
}
\label{tab:absolutePerformance}
\setlength\tabcolsep{4pt}
\resizebox{2\columnwidth}{!}{%
\begin{tabular}{lcc|cc|ccc|cc|cc|cc|cc}
\toprule
 & \multicolumn{2}{c}{\textbf{Initial}} & \multicolumn{2}{c}{\textbf{Resyn2}} & \multicolumn{3}{c}{\textbf{Simulated annealing}} & \multicolumn{2}{c}{\textbf{Standalone}} & \multicolumn{6}{c}{\textbf{\solution}} \\
 
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-8} \cmidrule(lr){9-10} \cmidrule(lr){11-16} 
\multirow{-2}{*}{\textbf{Design}} & Nodes & Depth & x$1$ & x$2$ & $B_{1k}$ & $B_{5k}$ & $B_{10k}$ & $S_{1k}$ & $S_{10k}$ & $ZS_{1k}$ & $ZS_{10k}$ & $F^R_{1k}$ & $F^R_{10k}$ & $F^A_{1k}$ & $F^A_{10k}$  \\ \midrule
apex1 &	1577 &	14  &	1201 & 1160	& 1091 &	1082 &	1082 &	1256 &	1177 &	1223 &	1211 & 	1148  &	1099 & 1150 &	1109 \\
bc0 & 1592 &	31 & 899 &	885	&	820	& 818	& 791 &		887 &		849 &		838 &		826 &		817 &		813 &		826	&	795	 \\
c1355 &	512	& 29 &	394 &	394 &		394	& 394	& 393	&	394 &		392 &		394	&	392 &		392 &		392 &		392 &		390  \\
c5315 &	1613	& 38 &	1289 &	1289 & 1254 & 1254	& 1254	& 1272 & 1268 &	1282 &	1274 &	1268 &	1265 &	1274 &1261  \\
c6288	& 2337	& 120 &	1870&	1870 &		1869 &	1869	& 1869 &		1870&		1870&		1872&		1870&		1870&		1870	&	1870	&	1870 \\
c7552	& 2198	&30	&	1433&	1417 &	1399&	1378&	1361&		1442&		1386&		1385&		1381&		1403&		1388&		1403&		1367 \\
dalu &	1735&	35 & 1052 &	1052 &		894&	894	&894	&	991	&	984	&	988	&	975	&	976	&	972	&	983	&	901	 \\
div & 57247 & 4372 & 40739 & 40716 & 20775 & 20740 & 20720 & 40068 & 39991 & 40881 & 37051 & 27891 & 22841 & 25871 & 20790 \\
i10	 &2273 &	58 &	1707&	1695	&	1685	&1674	&1662	&	1690&		1663&		1682&		1658&		1663&		1660&		1675&		1645 \\
k2&	2289&	22 &	1316&	1263 &		1280&	1242&	1230&		1467&		1464&		1490&		1425&		1409&		1369&		1418&		1359 \\
log2&	32060&	444	&	29302&	29259 &	29234&	29165&	29159&		30667	&	29375&		29434&		29371&		29429&		29328&		29332&		29250 \\
mainpla &	5346&	38 &	3583&	3522	&	3337&	3319&	3288&		3482&		3432&		3444	&	3414	&	3398&		3364&		3443&		3312 \\
max	& 2865 &	287	&	2832&	2831 &	2825&	2823&	2822&		286 5&		2859&		2853&		2850	&	2830	&	2830&		2834&		2819 \\
multiplier&	27062&	274	&	24554 &	24554 &	24360&	24360&	24360	&	25394&		24372&		24542&		24541	&	24416&		24368&		24641&		24368 \\
sin	& 5416&	225 &	5024&	5014	&	5006&	5004&	5003	&	5085&		5029	&	5036&		5042&		5033&		5025&		5036	&	5001 \\
sqrt &	24618&	5058 &	19437	&19437 &		19102&	19101	&19101&		19329	&	19288&		19385&		19322&		19402&		19351	&	19326	&	19121 \\
square&	18484&	250	&	16568&	16568 &	16253&	16252&	16252&		17044	&	17032	&	17011	&	16996	&	17092	&	17028&		17017&		16385 \\
\midrule
aes\_secworks & 40778 & 42 & 31195 & 30532 & 30668 & 30445	& 30186 & 31147	&	31243	&	30893&		30899		&31059	&	30714&		30438&		30437 \\
aes\_xcrypt & 45840 & 43 & 41720 & 40975& 42954&	42903	&42825 & 43338&		43074	&	43747&		43543&		43205&		42989&		43231	&	43035\\
bp\_be & 82514 & 86 & 78458	& 78402 &78176&	78012&	77926& 78308&		78591	&	78262	&	78487&		78211	&	78098&		78407&		78064\\
ethernet & 67164 & 34 & 64948 &	64872 &64844&	64821&	64813& 64942&		64932&		64968	&	65011&		64890&		64839	&	64870	&	64858 \\
jpeg & 114771 & 40 & 104235	& 104144& 102441&	102341&	 102320 & 103797	&	103465	&	102922	&	102616	&	102646	&	102710	&	102558	&	102441\\
picosoc & 82945 & 43 & 76806 &	76716 &76515&	76490&	76398& 77394	&	76747	&	76738	&	76698&		76753&		76598	&	76800	&	76715 \\
tinyRocket & 52315 & 80 & 41172	& 40981 &40793&	40674&	40717 & 40896	&	41005	&	40833	&	40820		&40954	&	40854&		40961&		40890\\
vga\_lcd & 105334 & 23 & 103630	& 103612& 103539&	103482&	103509& 103585	&	103635	&	103668	&	103647		&103679	&	103601	&	103618	&	103610 \\
wb\_conmax & 47840 & 24 & 44624	& 44544& 43910&	43859&	43648& 44651	&	44333	&	44090	&	43997		&44095	&	44075	&	43876	&	43926\\
\bottomrule
\end{tabular}%
}
\small {Subscript indicates number of calls to the evaluator (1k - 1000 calls)}
\end{table*}
